Virtual element methods for a class of fully nonlinear elliptic PDEs

We study virtual element discretizations of a well-known variational formulation in $H^2$ of Hamilton-Jacobi-Bellman and Isaacs equations with Cordes coefficients. We show that the use of $H^2$ conforming virtual element spaces leads to a relatively simple analysis, bypassing the need for discrete Miranda-Talenti estimates that typically arises when using nonconforming schemes. We investigate how the polynomial degree of projection operators, especially for lower order terms, affects both the error analysis and robustness of the proposed schemes. We also show the possibility of imposing weakly the Dirichlet boundary condition, which simplifies the implementation of the method in some virtual element codes. Our results are complemented by numerical experiments in which we compare the convergence of different variants of the scheme for some test problems.

==> results/A2/eps/A2IterDGvoronoi2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(8217,3034){\makebox(0,0)[r]{\strut{}level 6}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}DG m=2 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterDGvoronoi2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterDGvoronoi3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}DG m=3 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterDGvoronoi3-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterDGvoronoi4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}DG m=4 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterDGvoronoi4-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterDGvoronoi5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}DG m=5 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterDGvoronoi5-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM-1simplex2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) m=2 on simplex grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM-1simplex2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM-1simplex3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) m=3 on simplex grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM-1simplex3-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM-1simplex4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) m=4 on simplex grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM-1simplex4-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM-1simplex5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) m=5 on simplex grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM-1simplex5-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM-1voronoi2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(8217,3034){\makebox(0,0)[r]{\strut{}level 6}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) m=2 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM-1voronoi2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM-1voronoi3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) m=3 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM-1voronoi3-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM-1voronoi4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) m=4 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM-1voronoi4-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM-1voronoi5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) m=5 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM-1voronoi5-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM0voronoi2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(8217,3034){\makebox(0,0)[r]{\strut{}level 6}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m,m) m=2 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM0voronoi2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM0voronoi3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m,m) m=3 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM0voronoi3-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM0voronoi4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m,m) m=4 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM0voronoi4-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM0voronoi5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m,m) m=5 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM0voronoi5-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM1simplex2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) m=2 on simplex grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM1simplex2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM1simplex3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) m=3 on simplex grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM1simplex3-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM1simplex4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) m=4 on simplex grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM1simplex4-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM1simplex5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) m=5 on simplex grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM1simplex5-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM1voronoi2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(8217,3034){\makebox(0,0)[r]{\strut{}level 6}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) m=2 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM1voronoi2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM1voronoi3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) m=3 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM1voronoi3-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM1voronoi4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) m=4 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM1voronoi4-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM1voronoi5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) m=5 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM1voronoi5-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM2simplex2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) m=2 on simplex grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM2simplex2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM2simplex3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) m=3 on simplex grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM2simplex3-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM2simplex4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) m=4 on simplex grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM2simplex4-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM2simplex5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) m=5 on simplex grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM2simplex5-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM2voronoi2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(8217,3034){\makebox(0,0)[r]{\strut{}level 6}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) m=2 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM2voronoi2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM2voronoi3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) m=3 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM2voronoi3-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM2voronoi4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) m=4 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM2voronoi4-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEM2voronoi5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) m=5 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEM2voronoi5-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEMBnd0voronoi2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(8217,3034){\makebox(0,0)[r]{\strut{}level 6}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) m=2 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEMBnd0voronoi2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEMBnd0voronoi3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) m=3 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEMBnd0voronoi3-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEMBnd0voronoi4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) m=4 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEMBnd0voronoi4-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/A2IterVEMBnd0voronoi5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) m=5 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/A2IterVEMBnd0voronoi5-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/H1A2simplexEOC_vembnd-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1257){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2237){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3218){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4198){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/H1A2simplexEOC_vembnd-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/H1A2simplexEOC_vembnd1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1257){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2237){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3218){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4198){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/H1A2simplexEOC_vembnd1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/H1A2simplexEOC_vembnd2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1257){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2237){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3218){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4198){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/H1A2simplexEOC_vembnd2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/H1A2voronoiEOC_dg_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}DG m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}DG m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}DG m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}DG m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}DG vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/H1A2voronoiEOC_dg_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/H1A2voronoiEOC_vem-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/H1A2voronoiEOC_vem-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/H1A2voronoiEOC_vem1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/H1A2voronoiEOC_vem1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/H1A2voronoiEOC_vem2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/H1A2voronoiEOC_vem2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/H1A2voronoiEOC_vembnd-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/H1A2voronoiEOC_vembnd-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/H1A2voronoiEOC_vembnd0_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/H1A2voronoiEOC_vembnd0_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/H1A2voronoiEOC_vembnd1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/H1A2voronoiEOC_vembnd1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/H1A2voronoiEOC_vembnd2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/H1A2voronoiEOC_vembnd2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/H2A2simplexEOC_vembnd-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/H2A2simplexEOC_vembnd-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/H2A2simplexEOC_vembnd1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/H2A2simplexEOC_vembnd1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/H2A2simplexEOC_vembnd2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/H2A2simplexEOC_vembnd2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/H2A2voronoiEOC_dg_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}DG m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}DG m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}DG m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}DG m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}DG vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/H2A2voronoiEOC_dg_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/H2A2voronoiEOC_vem-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/H2A2voronoiEOC_vem-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/H2A2voronoiEOC_vem1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/H2A2voronoiEOC_vem1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/H2A2voronoiEOC_vem2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/H2A2voronoiEOC_vem2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/H2A2voronoiEOC_vembnd-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/H2A2voronoiEOC_vembnd-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/H2A2voronoiEOC_vembnd0_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/H2A2voronoiEOC_vembnd0_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/H2A2voronoiEOC_vembnd1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/H2A2voronoiEOC_vembnd1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/H2A2voronoiEOC_vembnd2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/H2A2voronoiEOC_vembnd2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/L2A2simplexEOC_vembnd-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/L2A2simplexEOC_vembnd-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/L2A2simplexEOC_vembnd1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/L2A2simplexEOC_vembnd1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/L2A2simplexEOC_vembnd2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/L2A2simplexEOC_vembnd2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/L2A2voronoiEOC_dg_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,1159){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1943){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3512){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4296){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}DG m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}DG m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}DG m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}DG m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}DG vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/L2A2voronoiEOC_dg_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/L2A2voronoiEOC_vem-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,1159){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1943){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3512){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4296){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/L2A2voronoiEOC_vem-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/L2A2voronoiEOC_vem1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,1159){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1943){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3512){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4296){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/L2A2voronoiEOC_vem1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/L2A2voronoiEOC_vem2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,1159){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1943){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3512){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4296){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/L2A2voronoiEOC_vem2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/L2A2voronoiEOC_vembnd-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,1159){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1943){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3512){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4296){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/L2A2voronoiEOC_vembnd-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/L2A2voronoiEOC_vembnd0_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,1159){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1943){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3512){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4296){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/L2A2voronoiEOC_vembnd0_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/L2A2voronoiEOC_vembnd1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,1159){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1943){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3512){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4296){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/L2A2voronoiEOC_vembnd1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/L2A2voronoiEOC_vembnd2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,1159){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1943){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3512){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4296){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/L2A2voronoiEOC_vembnd2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/dgA2simplex_20.tex <==
\begin{tabular}{rrr}
\hline
   $H^2$ &   $H^1$ &   $L^2$ \\
\hline
    0.37 &    0.41 &    0.45 \\
    0.76 &    0.83 &    0.9  \\
    1.28 &    1.4  &    1.43 \\
    1.5  &    1.78 &    1.79 \\
    1.35 &    1.93 &    1.94 \\
\hline
\end{tabular}

==> results/A2/eps/dgA2simplex_30.tex <==
\begin{tabular}{rrr}
\hline
   $H^2$ &   $H^1$ &   $L^2$ \\
\hline
    1.66 &    2.75 &    2.88 \\
    2.11 &    3.15 &    3.25 \\
    2.43 &    3.4  &    3.43 \\
    2.44 &    3.2  &    3.08 \\
    2.28 &    2.64 &    2.46 \\
\hline
\end{tabular}

==> results/A2/eps/dgA2simplex_40.tex <==
\begin{tabular}{rrr}
\hline
   $H^2$ &   $H^1$ &   $L^2$ \\
\hline
    2.62 &    3.6  &    4.54 \\
    3.09 &    4.09 &    4.82 \\
    3.38 &    4.41 &    4.87 \\
    3.38 &    4.43 &    4.63 \\
\hline
\end{tabular}

==> results/A2/eps/dgA2simplex_50.tex <==
\begin{tabular}{rrr}
\hline
   $H^2$ &   $H^1$ &   $L^2$ \\
\hline
    3.98 &    5.04 &    6.16 \\
    4.07 &    5.08 &    5.91 \\
    4.04 &    5.03 &    5.32 \\
\hline
\end{tabular}

==> results/A2/eps/dgA2voronoi_20.tex <==
\begin{tabular}{rrr}
\hline
   $H^2$ &   $H^1$ &   $L^2$ \\
\hline
    0.69 &    0.7  &    0.62 \\
    1.16 &    1.23 &    1.19 \\
    1.48 &    1.68 &    1.63 \\
    1.4  &    1.88 &    1.9  \\
    1.22 &    1.93 &    1.92 \\
\hline
\end{tabular}

==> results/A2/eps/dgA2voronoi_30.tex <==
\begin{tabular}{rrr}
\hline
   $H^2$ &   $H^1$ &   $L^2$ \\
\hline
    2.52 &    3.71 &    3.89 \\
    2.27 &    3.5  &    4.12 \\
    2.13 &    3.34 &    3.71 \\
    2.03 &    2.43 &    1.57 \\
\hline
\end{tabular}

==> results/A2/eps/dgA2voronoi_40.tex <==
\begin{tabular}{rrr}
\hline
   $H^2$ &   $H^1$ &   $L^2$ \\
\hline
    3.54 &    4.85 &    6.32 \\
    3.06 &    4.11 &    5.3  \\
    3.02 &    4.02 &    4.83 \\
    3    &    4.01 &    4.42 \\
\hline
\end{tabular}

==> results/A2/eps/dgA2voronoi_50.tex <==
\begin{tabular}{rrr}
\hline
   $H^2$ &   $H^1$ &   $L^2$ \\
\hline
    4.19 &    5.27 &    6.5  \\
    4    &    4.95 &    5.51 \\
    3.97 &    4.95 &    4.97 \\
\hline
\end{tabular}

==> results/A2/eps/starA2simplexEOC_dg_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2459,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3924,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5388,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6853,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}DG m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}DG m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}DG m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}DG m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}DG vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/starA2simplexEOC_dg_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/starA2simplexEOC_vem-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2459,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3924,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5388,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6853,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/starA2simplexEOC_vem-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/starA2simplexEOC_vem1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2459,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3924,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5388,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6853,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/starA2simplexEOC_vem1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/starA2simplexEOC_vem2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2459,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3924,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5388,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6853,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/starA2simplexEOC_vem2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/starA2simplexEOC_vembnd-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2459,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3924,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5388,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6853,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/starA2simplexEOC_vembnd-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/starA2simplexEOC_vembnd0_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2459,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3924,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5388,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6853,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/starA2simplexEOC_vembnd0_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/starA2simplexEOC_vembnd1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2459,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3924,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5388,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6853,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/starA2simplexEOC_vembnd1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/starA2simplexEOC_vembnd2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2459,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3924,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5388,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6853,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/starA2simplexEOC_vembnd2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/starA2voronoiEOC_dg_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1257){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2237){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3218){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4198){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}DG m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}DG m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}DG m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}DG m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}DG vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/starA2voronoiEOC_dg_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/starA2voronoiEOC_vem-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/starA2voronoiEOC_vem-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/starA2voronoiEOC_vem1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/starA2voronoiEOC_vem1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/starA2voronoiEOC_vem2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/starA2voronoiEOC_vem2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/starA2voronoiEOC_vembnd-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/starA2voronoiEOC_vembnd-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/starA2voronoiEOC_vembnd0_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/starA2voronoiEOC_vembnd0_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/starA2voronoiEOC_vembnd1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/starA2voronoiEOC_vembnd1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/starA2voronoiEOC_vembnd2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/starA2voronoiEOC_vembnd2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/vem0A2simplexEOCH1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(692,767){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(692,1159){\makebox(0,0)[r]{\strut{}1.0}}%
      \csname LTb\endcsname%%
      \put(692,1551){\makebox(0,0)[r]{\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(692,1943){\makebox(0,0)[r]{\strut{}2.0}}%
      \csname LTb\endcsname%%
      \put(692,2335){\makebox(0,0)[r]{\strut{}2.5}}%
      \csname LTb\endcsname%%
      \put(692,2727){\makebox(0,0)[r]{\strut{}3.0}}%
      \csname LTb\endcsname%%
      \put(692,3120){\makebox(0,0)[r]{\strut{}3.5}}%
      \csname LTb\endcsname%%
      \put(692,3512){\makebox(0,0)[r]{\strut{}4.0}}%
      \csname LTb\endcsname%%
      \put(692,3904){\makebox(0,0)[r]{\strut{}4.5}}%
      \csname LTb\endcsname%%
      \put(692,4296){\makebox(0,0)[r]{\strut{}5.0}}%
      \csname LTb\endcsname%%
      \put(692,4688){\makebox(0,0)[r]{\strut{}5.5}}%
      \csname LTb\endcsname%%
      \put(793,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2674,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4555,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6436,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(7517,4472){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(7517,4233){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(7517,3993){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(7517,3753){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ eoc}}}%
      \csname LTb\endcsname%%
      \put(4555,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4555,5380){\makebox(0,0){\strut{}Simplex grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/vem0A2simplexEOCH1-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/vem0A2simplexEOCH2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(692,767){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(692,1257){\makebox(0,0)[r]{\strut{}1.0}}%
      \csname LTb\endcsname%%
      \put(692,1747){\makebox(0,0)[r]{\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(692,2237){\makebox(0,0)[r]{\strut{}2.0}}%
      \csname LTb\endcsname%%
      \put(692,2727){\makebox(0,0)[r]{\strut{}2.5}}%
      \csname LTb\endcsname%%
      \put(692,3218){\makebox(0,0)[r]{\strut{}3.0}}%
      \csname LTb\endcsname%%
      \put(692,3708){\makebox(0,0)[r]{\strut{}3.5}}%
      \csname LTb\endcsname%%
      \put(692,4198){\makebox(0,0)[r]{\strut{}4.0}}%
      \csname LTb\endcsname%%
      \put(692,4688){\makebox(0,0)[r]{\strut{}4.5}}%
      \csname LTb\endcsname%%
      \put(793,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2674,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4555,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6436,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(7517,4472){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(7517,4233){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(7517,3993){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(7517,3753){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ eoc}}}%
      \csname LTb\endcsname%%
      \put(4555,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4555,5380){\makebox(0,0){\strut{}Simplex grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/vem0A2simplexEOCH2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/vem0A2simplexEOCL2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(692,767){\makebox(0,0)[r]{\strut{}0.0}}%
      \csname LTb\endcsname%%
      \put(692,1327){\makebox(0,0)[r]{\strut{}1.0}}%
      \csname LTb\endcsname%%
      \put(692,1887){\makebox(0,0)[r]{\strut{}2.0}}%
      \csname LTb\endcsname%%
      \put(692,2447){\makebox(0,0)[r]{\strut{}3.0}}%
      \csname LTb\endcsname%%
      \put(692,3007){\makebox(0,0)[r]{\strut{}4.0}}%
      \csname LTb\endcsname%%
      \put(692,3568){\makebox(0,0)[r]{\strut{}5.0}}%
      \csname LTb\endcsname%%
      \put(692,4128){\makebox(0,0)[r]{\strut{}6.0}}%
      \csname LTb\endcsname%%
      \put(692,4688){\makebox(0,0)[r]{\strut{}7.0}}%
      \csname LTb\endcsname%%
      \put(793,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2674,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4555,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6436,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(7517,4472){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(7517,4233){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(7517,3993){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(7517,3753){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ eoc}}}%
      \csname LTb\endcsname%%
      \put(4555,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4555,5380){\makebox(0,0){\strut{}Simplex grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/vem0A2simplexEOCL2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/vem0A2simplexEOCstar.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(692,767){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(692,1257){\makebox(0,0)[r]{\strut{}1.0}}%
      \csname LTb\endcsname%%
      \put(692,1747){\makebox(0,0)[r]{\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(692,2237){\makebox(0,0)[r]{\strut{}2.0}}%
      \csname LTb\endcsname%%
      \put(692,2727){\makebox(0,0)[r]{\strut{}2.5}}%
      \csname LTb\endcsname%%
      \put(692,3218){\makebox(0,0)[r]{\strut{}3.0}}%
      \csname LTb\endcsname%%
      \put(692,3708){\makebox(0,0)[r]{\strut{}3.5}}%
      \csname LTb\endcsname%%
      \put(692,4198){\makebox(0,0)[r]{\strut{}4.0}}%
      \csname LTb\endcsname%%
      \put(692,4688){\makebox(0,0)[r]{\strut{}4.5}}%
      \csname LTb\endcsname%%
      \put(793,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2674,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4555,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6436,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(7517,4472){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(7517,4233){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(7517,3993){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(7517,3753){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ eoc}}}%
      \csname LTb\endcsname%%
      \put(4555,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4555,5380){\makebox(0,0){\strut{}Simplex grid $\|\cdot\|_\star$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/vem0A2simplexEOCstar-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/vem0A2simplexErrstar.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}Simplex grid $\|\cdot\|_\star$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/vem0A2simplexErrstar-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/vem0A2voronoiEOCH1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(692,767){\makebox(0,0)[r]{\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(692,1257){\makebox(0,0)[r]{\strut{}2.0}}%
      \csname LTb\endcsname%%
      \put(692,1747){\makebox(0,0)[r]{\strut{}2.5}}%
      \csname LTb\endcsname%%
      \put(692,2237){\makebox(0,0)[r]{\strut{}3.0}}%
      \csname LTb\endcsname%%
      \put(692,2727){\makebox(0,0)[r]{\strut{}3.5}}%
      \csname LTb\endcsname%%
      \put(692,3218){\makebox(0,0)[r]{\strut{}4.0}}%
      \csname LTb\endcsname%%
      \put(692,3708){\makebox(0,0)[r]{\strut{}4.5}}%
      \csname LTb\endcsname%%
      \put(692,4198){\makebox(0,0)[r]{\strut{}5.0}}%
      \csname LTb\endcsname%%
      \put(692,4688){\makebox(0,0)[r]{\strut{}5.5}}%
      \csname LTb\endcsname%%
      \put(793,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(3301,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(5809,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(7517,4472){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(7517,4233){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(7517,3993){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(7517,3753){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ eoc}}}%
      \csname LTb\endcsname%%
      \put(4555,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4555,5380){\makebox(0,0){\strut{}Voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/vem0A2voronoiEOCH1-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/vem0A2voronoiEOCH2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(692,767){\makebox(0,0)[r]{\strut{}1.0}}%
      \csname LTb\endcsname%%
      \put(692,1327){\makebox(0,0)[r]{\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(692,1887){\makebox(0,0)[r]{\strut{}2.0}}%
      \csname LTb\endcsname%%
      \put(692,2447){\makebox(0,0)[r]{\strut{}2.5}}%
      \csname LTb\endcsname%%
      \put(692,3007){\makebox(0,0)[r]{\strut{}3.0}}%
      \csname LTb\endcsname%%
      \put(692,3568){\makebox(0,0)[r]{\strut{}3.5}}%
      \csname LTb\endcsname%%
      \put(692,4128){\makebox(0,0)[r]{\strut{}4.0}}%
      \csname LTb\endcsname%%
      \put(692,4688){\makebox(0,0)[r]{\strut{}4.5}}%
      \csname LTb\endcsname%%
      \put(793,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(3301,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(5809,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(7517,4472){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(7517,4233){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(7517,3993){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(7517,3753){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ eoc}}}%
      \csname LTb\endcsname%%
      \put(4555,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4555,5380){\makebox(0,0){\strut{}Voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/vem0A2voronoiEOCH2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/vem0A2voronoiEOCL2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(692,767){\makebox(0,0)[r]{\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(692,1202){\makebox(0,0)[r]{\strut{}2.0}}%
      \csname LTb\endcsname%%
      \put(692,1638){\makebox(0,0)[r]{\strut{}2.5}}%
      \csname LTb\endcsname%%
      \put(692,2074){\makebox(0,0)[r]{\strut{}3.0}}%
      \csname LTb\endcsname%%
      \put(692,2509){\makebox(0,0)[r]{\strut{}3.5}}%
      \csname LTb\endcsname%%
      \put(692,2945){\makebox(0,0)[r]{\strut{}4.0}}%
      \csname LTb\endcsname%%
      \put(692,3381){\makebox(0,0)[r]{\strut{}4.5}}%
      \csname LTb\endcsname%%
      \put(692,3817){\makebox(0,0)[r]{\strut{}5.0}}%
      \csname LTb\endcsname%%
      \put(692,4252){\makebox(0,0)[r]{\strut{}5.5}}%
      \csname LTb\endcsname%%
      \put(692,4688){\makebox(0,0)[r]{\strut{}6.0}}%
      \csname LTb\endcsname%%
      \put(793,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(3301,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(5809,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(7517,4472){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(7517,4233){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(7517,3993){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(7517,3753){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ eoc}}}%
      \csname LTb\endcsname%%
      \put(4555,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4555,5380){\makebox(0,0){\strut{}Voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/vem0A2voronoiEOCL2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/vem0A2voronoiEOCstar.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(692,767){\makebox(0,0)[r]{\strut{}1.0}}%
      \csname LTb\endcsname%%
      \put(692,1327){\makebox(0,0)[r]{\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(692,1887){\makebox(0,0)[r]{\strut{}2.0}}%
      \csname LTb\endcsname%%
      \put(692,2447){\makebox(0,0)[r]{\strut{}2.5}}%
      \csname LTb\endcsname%%
      \put(692,3007){\makebox(0,0)[r]{\strut{}3.0}}%
      \csname LTb\endcsname%%
      \put(692,3568){\makebox(0,0)[r]{\strut{}3.5}}%
      \csname LTb\endcsname%%
      \put(692,4128){\makebox(0,0)[r]{\strut{}4.0}}%
      \csname LTb\endcsname%%
      \put(692,4688){\makebox(0,0)[r]{\strut{}4.5}}%
      \csname LTb\endcsname%%
      \put(793,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(3301,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(5809,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(7517,4472){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(7517,4233){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(7517,3993){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(7517,3753){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ eoc}}}%
      \csname LTb\endcsname%%
      \put(4555,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4555,5380){\makebox(0,0){\strut{}Voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/vem0A2voronoiEOCstar-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A2/eps/vem0A2voronoiErrstar.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}Voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A2/eps/vem0A2voronoiErrstar-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterDGsimplex2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(8217,3034){\makebox(0,0)[r]{\strut{}level 6}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}DG m=2 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterDGsimplex2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterDGsimplex3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}DG m=3 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterDGsimplex3-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterDGsimplex4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}DG m=4 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterDGsimplex4-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterDGsimplex5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}DG m=5 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterDGsimplex5-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterDGvoronoi2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}DG m=2 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterDGvoronoi2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterDGvoronoi3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}DG m=3 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterDGvoronoi3-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterDGvoronoi4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}DG m=4 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterDGvoronoi4-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterDGvoronoi5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}DG m=5 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterDGvoronoi5-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM-1simplex2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(8217,3034){\makebox(0,0)[r]{\strut{}level 6}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) m=2 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM-1simplex2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM-1simplex3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) m=3 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM-1simplex3-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM-1simplex4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) m=4 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM-1simplex4-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM-1simplex5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) m=5 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM-1simplex5-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM-1voronoi2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) m=2 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM-1voronoi2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM-1voronoi3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) m=3 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM-1voronoi3-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM-1voronoi4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) m=4 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM-1voronoi4-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM-1voronoi5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) m=5 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM-1voronoi5-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM0simplex2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(8217,3034){\makebox(0,0)[r]{\strut{}level 6}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m,m) m=2 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM0simplex2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM0simplex3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m,m) m=3 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM0simplex3-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM0simplex4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m,m) m=4 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM0simplex4-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM0simplex5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m,m) m=5 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM0simplex5-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM0voronoi2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m,m) m=2 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM0voronoi2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM0voronoi3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m,m) m=3 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM0voronoi3-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM0voronoi4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m,m) m=4 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM0voronoi4-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM0voronoi5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m,m,m) m=5 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM0voronoi5-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM1simplex2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(8217,3034){\makebox(0,0)[r]{\strut{}level 6}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) m=2 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM1simplex2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM1simplex3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) m=3 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM1simplex3-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM1simplex4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) m=4 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM1simplex4-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM1simplex5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) m=5 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM1simplex5-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM1voronoi2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) m=2 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM1voronoi2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM1voronoi3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) m=3 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM1voronoi3-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM1voronoi4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) m=4 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM1voronoi4-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM1voronoi5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) m=5 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM1voronoi5-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM2simplex2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(8217,3034){\makebox(0,0)[r]{\strut{}level 6}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) m=2 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM2simplex2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM2simplex3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) m=3 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM2simplex3-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM2simplex4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) m=4 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM2simplex4-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM2simplex5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) m=5 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM2simplex5-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM2voronoi2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) m=2 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM2voronoi2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM2voronoi3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) m=3 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM2voronoi3-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM2voronoi4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) m=4 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM2voronoi4-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEM2voronoi5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) m=5 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEM2voronoi5-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEMBnd0simplex2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(8217,3034){\makebox(0,0)[r]{\strut{}level 6}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) m=2 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEMBnd0simplex2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEMBnd0simplex3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) m=3 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEMBnd0simplex3-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEMBnd0simplex4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) m=4 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEMBnd0simplex4-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEMBnd0simplex5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) m=5 }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEMBnd0simplex5-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEMBnd0voronoi2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) m=2 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEMBnd0voronoi2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEMBnd0voronoi3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(8217,3274){\makebox(0,0)[r]{\strut{}level 5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) m=3 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEMBnd0voronoi3-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEMBnd0voronoi4.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(8217,3514){\makebox(0,0)[r]{\strut{}level 4}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) m=4 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEMBnd0voronoi4-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/A3IterVEMBnd0voronoi5.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1095,767){\makebox(0,0)[r]{\strut{}$1\times10^{-14}$}}%
      \csname LTb\endcsname%%
      \put(1095,1327){\makebox(0,0)[r]{\strut{}$1\times10^{-12}$}}%
      \csname LTb\endcsname%%
      \put(1095,1887){\makebox(0,0)[r]{\strut{}$1\times10^{-10}$}}%
      \csname LTb\endcsname%%
      \put(1095,2447){\makebox(0,0)[r]{\strut{}$1\times10^{-8}$}}%
      \csname LTb\endcsname%%
      \put(1095,3007){\makebox(0,0)[r]{\strut{}$1\times10^{-6}$}}%
      \csname LTb\endcsname%%
      \put(1095,3568){\makebox(0,0)[r]{\strut{}$0.0001$}}%
      \csname LTb\endcsname%%
      \put(1095,4128){\makebox(0,0)[r]{\strut{}$0.01$}}%
      \csname LTb\endcsname%%
      \put(1095,4688){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(1196,527){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2213,527){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(3231,527){\makebox(0,0){\strut{}$3$}}%
      \csname LTb\endcsname%%
      \put(4248,527){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%%
      \put(5265,527){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%%
      \put(6283,527){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%%
      \put(7300,527){\makebox(0,0){\strut{}$7$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$8$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(8217,4472){\makebox(0,0)[r]{\strut{}tolerance 1e-9}}%
      \csname LTb\endcsname%%
      \put(8217,4233){\makebox(0,0)[r]{\strut{}level 1}}%
      \csname LTb\endcsname%%
      \put(8217,3993){\makebox(0,0)[r]{\strut{}level 2}}%
      \csname LTb\endcsname%%
      \put(8217,3753){\makebox(0,0)[r]{\strut{}level 3}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}relative residual in dual norm}}}%
      \csname LTb\endcsname%%
      \put(4757,167){\makebox(0,0){\strut{}iterations}}%
      \csname LTb\endcsname%%
      \put(4757,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) m=5 on voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/A3IterVEMBnd0voronoi5-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H1A3simplexEOC_dg_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1257){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2237){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3218){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4198){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2459,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3924,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5388,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6853,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}DG m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}DG m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}DG m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}DG m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}DG vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H1A3simplexEOC_dg_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H1A3simplexEOC_vem-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1257){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2237){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3218){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4198){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H1A3simplexEOC_vem-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H1A3simplexEOC_vem1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H1A3simplexEOC_vem1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H1A3simplexEOC_vem2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H1A3simplexEOC_vem2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H1A3simplexEOC_vembnd-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1257){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2237){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3218){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4198){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H1A3simplexEOC_vembnd-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H1A3simplexEOC_vembnd0_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H1A3simplexEOC_vembnd0_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H1A3simplexEOC_vembnd1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H1A3simplexEOC_vembnd1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H1A3simplexEOC_vembnd2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H1A3simplexEOC_vembnd2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H1A3voronoiEOC_dg_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}DG m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}DG m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}DG m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}DG m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}DG vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H1A3voronoiEOC_dg_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H1A3voronoiEOC_vem-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H1A3voronoiEOC_vem-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H1A3voronoiEOC_vem1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1257){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2237){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3218){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4198){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H1A3voronoiEOC_vem1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H1A3voronoiEOC_vem2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1257){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2237){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3218){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4198){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H1A3voronoiEOC_vem2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H1A3voronoiEOC_vembnd-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H1A3voronoiEOC_vembnd-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H1A3voronoiEOC_vembnd0_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1257){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2237){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3218){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4198){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H1A3voronoiEOC_vembnd0_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H1A3voronoiEOC_vembnd1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1257){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2237){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3218){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4198){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H1A3voronoiEOC_vembnd1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H1A3voronoiEOC_vembnd2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1257){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2237){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3218){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4198){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H1A3voronoiEOC_vembnd2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H2A3simplexEOC_dg_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2459,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3924,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5388,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6853,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}DG m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}DG m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}DG m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}DG m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}DG vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H2A3simplexEOC_dg_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H2A3simplexEOC_vem-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H2A3simplexEOC_vem-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H2A3simplexEOC_vem1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H2A3simplexEOC_vem1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H2A3simplexEOC_vem2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H2A3simplexEOC_vem2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H2A3simplexEOC_vembnd-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H2A3simplexEOC_vembnd-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H2A3simplexEOC_vembnd0_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H2A3simplexEOC_vembnd0_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H2A3simplexEOC_vembnd1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H2A3simplexEOC_vembnd1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H2A3simplexEOC_vembnd2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H2A3simplexEOC_vembnd2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H2A3voronoiEOC_dg_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}DG m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}DG m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}DG m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}DG m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}DG vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H2A3voronoiEOC_dg_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H2A3voronoiEOC_vem-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H2A3voronoiEOC_vem-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H2A3voronoiEOC_vem1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H2A3voronoiEOC_vem1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H2A3voronoiEOC_vem2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H2A3voronoiEOC_vem2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H2A3voronoiEOC_vembnd-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H2A3voronoiEOC_vembnd-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H2A3voronoiEOC_vembnd0_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H2A3voronoiEOC_vembnd0_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H2A3voronoiEOC_vembnd1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H2A3voronoiEOC_vembnd1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/H2A3voronoiEOC_vembnd2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/H2A3voronoiEOC_vembnd2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/L2A3simplexEOC_dg_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-09}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2459,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3924,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5388,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6853,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}DG m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}DG m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}DG m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}DG m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}DG vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/L2A3simplexEOC_dg_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/L2A3simplexEOC_vem-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-09}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/L2A3simplexEOC_vem-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/L2A3simplexEOC_vem1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-09}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/L2A3simplexEOC_vem1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/L2A3simplexEOC_vem2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-09}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/L2A3simplexEOC_vem2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/L2A3simplexEOC_vembnd-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-09}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/L2A3simplexEOC_vembnd-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/L2A3simplexEOC_vembnd0_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-09}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/L2A3simplexEOC_vembnd0_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/L2A3simplexEOC_vembnd1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-09}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/L2A3simplexEOC_vembnd1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/L2A3simplexEOC_vembnd2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-09}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/L2A3simplexEOC_vembnd2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/L2A3voronoiEOC_dg_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-10}}%
      \csname LTb\endcsname%%
      \put(894,1551){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,2335){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,3120){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3904){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}DG m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}DG m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}DG m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}DG m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}DG vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/L2A3voronoiEOC_dg_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/L2A3voronoiEOC_vem-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-10}}%
      \csname LTb\endcsname%%
      \put(894,1551){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,2335){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,3120){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3904){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/L2A3voronoiEOC_vem-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/L2A3voronoiEOC_vem1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-10}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-09}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/L2A3voronoiEOC_vem1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/L2A3voronoiEOC_vem2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-10}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-09}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/L2A3voronoiEOC_vem2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/L2A3voronoiEOC_vembnd-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-10}}%
      \csname LTb\endcsname%%
      \put(894,1551){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,2335){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,3120){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3904){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/L2A3voronoiEOC_vembnd-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/L2A3voronoiEOC_vembnd0_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-10}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-09}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/L2A3voronoiEOC_vembnd0_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/L2A3voronoiEOC_vembnd1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-10}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-09}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/L2A3voronoiEOC_vembnd1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/L2A3voronoiEOC_vembnd2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-10}}%
      \csname LTb\endcsname%%
      \put(894,1202){\makebox(0,0)[r]{\strut{}1e-09}}%
      \csname LTb\endcsname%%
      \put(894,1638){\makebox(0,0)[r]{\strut{}1e-08}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,2509){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2945){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3817){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,4252){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/L2A3voronoiEOC_vembnd2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/starA3simplexEOC_dg_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2459,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3924,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5388,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6853,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}DG m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}DG m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}DG m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}DG m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}DG vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/starA3simplexEOC_dg_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/starA3simplexEOC_vem-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/starA3simplexEOC_vem-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/starA3simplexEOC_vem1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/starA3simplexEOC_vem1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/starA3simplexEOC_vem2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/starA3simplexEOC_vem2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/starA3simplexEOC_vembnd-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/starA3simplexEOC_vembnd-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/starA3simplexEOC_vembnd0_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/starA3simplexEOC_vembnd0_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/starA3simplexEOC_vembnd1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/starA3simplexEOC_vembnd1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/starA3simplexEOC_vembnd2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/starA3simplexEOC_vembnd2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/starA3voronoiEOC_dg_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1327){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,1887){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2447){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3007){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,3568){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4128){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}DG m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}DG m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}DG m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}DG m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}DG vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/starA3voronoiEOC_dg_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/starA3voronoiEOC_vem-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/starA3voronoiEOC_vem-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/starA3voronoiEOC_vem1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/starA3voronoiEOC_vem1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/starA3voronoiEOC_vem2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/starA3voronoiEOC_vem2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/starA3voronoiEOC_vembnd-1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m-1,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m-1,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/starA3voronoiEOC_vembnd-1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/starA3voronoiEOC_vembnd0_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m,m,m) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/starA3voronoiEOC_vembnd0_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/starA3voronoiEOC_vembnd1_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-1,m-1,m-1) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-1,m-1,m-1) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/starA3voronoiEOC_vembnd1_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/starA3voronoiEOC_vembnd2_vem0.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2660){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,2420){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM-Weak(m-2,m-2,m-2) m=5}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}VEM-Weak(m-2,m-2,m-2) vs VEM(m,m,m)}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/starA3voronoiEOC_vembnd2_vem0-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/vem0A3simplexEOCH1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(692,767){\makebox(0,0)[r]{\strut{}1.0}}%
      \csname LTb\endcsname%%
      \put(692,1202){\makebox(0,0)[r]{\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(692,1638){\makebox(0,0)[r]{\strut{}2.0}}%
      \csname LTb\endcsname%%
      \put(692,2074){\makebox(0,0)[r]{\strut{}2.5}}%
      \csname LTb\endcsname%%
      \put(692,2509){\makebox(0,0)[r]{\strut{}3.0}}%
      \csname LTb\endcsname%%
      \put(692,2945){\makebox(0,0)[r]{\strut{}3.5}}%
      \csname LTb\endcsname%%
      \put(692,3381){\makebox(0,0)[r]{\strut{}4.0}}%
      \csname LTb\endcsname%%
      \put(692,3817){\makebox(0,0)[r]{\strut{}4.5}}%
      \csname LTb\endcsname%%
      \put(692,4252){\makebox(0,0)[r]{\strut{}5.0}}%
      \csname LTb\endcsname%%
      \put(692,4688){\makebox(0,0)[r]{\strut{}5.5}}%
      \csname LTb\endcsname%%
      \put(793,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3301,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5809,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(7517,4472){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(7517,4233){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(7517,3993){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(7517,3753){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ eoc}}}%
      \csname LTb\endcsname%%
      \put(4555,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4555,5380){\makebox(0,0){\strut{}Simplex grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/vem0A3simplexEOCH1-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/vem0A3simplexEOCH2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(692,767){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(692,1257){\makebox(0,0)[r]{\strut{}1.0}}%
      \csname LTb\endcsname%%
      \put(692,1747){\makebox(0,0)[r]{\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(692,2237){\makebox(0,0)[r]{\strut{}2.0}}%
      \csname LTb\endcsname%%
      \put(692,2727){\makebox(0,0)[r]{\strut{}2.5}}%
      \csname LTb\endcsname%%
      \put(692,3218){\makebox(0,0)[r]{\strut{}3.0}}%
      \csname LTb\endcsname%%
      \put(692,3708){\makebox(0,0)[r]{\strut{}3.5}}%
      \csname LTb\endcsname%%
      \put(692,4198){\makebox(0,0)[r]{\strut{}4.0}}%
      \csname LTb\endcsname%%
      \put(692,4688){\makebox(0,0)[r]{\strut{}4.5}}%
      \csname LTb\endcsname%%
      \put(793,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3301,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5809,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(7517,4472){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(7517,4233){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(7517,3993){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(7517,3753){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ eoc}}}%
      \csname LTb\endcsname%%
      \put(4555,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4555,5380){\makebox(0,0){\strut{}Simplex grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/vem0A3simplexEOCH2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/vem0A3simplexEOCL2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(692,767){\makebox(0,0)[r]{\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(692,1159){\makebox(0,0)[r]{\strut{}2.0}}%
      \csname LTb\endcsname%%
      \put(692,1551){\makebox(0,0)[r]{\strut{}2.5}}%
      \csname LTb\endcsname%%
      \put(692,1943){\makebox(0,0)[r]{\strut{}3.0}}%
      \csname LTb\endcsname%%
      \put(692,2335){\makebox(0,0)[r]{\strut{}3.5}}%
      \csname LTb\endcsname%%
      \put(692,2727){\makebox(0,0)[r]{\strut{}4.0}}%
      \csname LTb\endcsname%%
      \put(692,3120){\makebox(0,0)[r]{\strut{}4.5}}%
      \csname LTb\endcsname%%
      \put(692,3512){\makebox(0,0)[r]{\strut{}5.0}}%
      \csname LTb\endcsname%%
      \put(692,3904){\makebox(0,0)[r]{\strut{}5.5}}%
      \csname LTb\endcsname%%
      \put(692,4296){\makebox(0,0)[r]{\strut{}6.0}}%
      \csname LTb\endcsname%%
      \put(692,4688){\makebox(0,0)[r]{\strut{}6.5}}%
      \csname LTb\endcsname%%
      \put(793,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3301,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5809,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(7517,4472){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(7517,4233){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(7517,3993){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(7517,3753){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ eoc}}}%
      \csname LTb\endcsname%%
      \put(4555,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4555,5380){\makebox(0,0){\strut{}Simplex grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/vem0A3simplexEOCL2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/vem0A3simplexEOCstar.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(692,767){\makebox(0,0)[r]{\strut{}0.5}}%
      \csname LTb\endcsname%%
      \put(692,1257){\makebox(0,0)[r]{\strut{}1.0}}%
      \csname LTb\endcsname%%
      \put(692,1747){\makebox(0,0)[r]{\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(692,2237){\makebox(0,0)[r]{\strut{}2.0}}%
      \csname LTb\endcsname%%
      \put(692,2727){\makebox(0,0)[r]{\strut{}2.5}}%
      \csname LTb\endcsname%%
      \put(692,3218){\makebox(0,0)[r]{\strut{}3.0}}%
      \csname LTb\endcsname%%
      \put(692,3708){\makebox(0,0)[r]{\strut{}3.5}}%
      \csname LTb\endcsname%%
      \put(692,4198){\makebox(0,0)[r]{\strut{}4.0}}%
      \csname LTb\endcsname%%
      \put(692,4688){\makebox(0,0)[r]{\strut{}4.5}}%
      \csname LTb\endcsname%%
      \put(793,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3301,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5809,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(7517,4472){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(7517,4233){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(7517,3993){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(7517,3753){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ eoc}}}%
      \csname LTb\endcsname%%
      \put(4555,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4555,5380){\makebox(0,0){\strut{}Simplex grid $\|\cdot\|_\star$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/vem0A3simplexEOCstar-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/vem0A3simplexErrstar.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}Simplex grid $\|\cdot\|_\star$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/vem0A3simplexErrstar-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/vem0A3voronoiEOCH1.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(692,767){\makebox(0,0)[r]{\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(692,1202){\makebox(0,0)[r]{\strut{}2.0}}%
      \csname LTb\endcsname%%
      \put(692,1638){\makebox(0,0)[r]{\strut{}2.5}}%
      \csname LTb\endcsname%%
      \put(692,2074){\makebox(0,0)[r]{\strut{}3.0}}%
      \csname LTb\endcsname%%
      \put(692,2509){\makebox(0,0)[r]{\strut{}3.5}}%
      \csname LTb\endcsname%%
      \put(692,2945){\makebox(0,0)[r]{\strut{}4.0}}%
      \csname LTb\endcsname%%
      \put(692,3381){\makebox(0,0)[r]{\strut{}4.5}}%
      \csname LTb\endcsname%%
      \put(692,3817){\makebox(0,0)[r]{\strut{}5.0}}%
      \csname LTb\endcsname%%
      \put(692,4252){\makebox(0,0)[r]{\strut{}5.5}}%
      \csname LTb\endcsname%%
      \put(692,4688){\makebox(0,0)[r]{\strut{}6.0}}%
      \csname LTb\endcsname%%
      \put(793,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(3301,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(5809,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(7517,4472){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(7517,4233){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(7517,3993){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(7517,3753){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ eoc}}}%
      \csname LTb\endcsname%%
      \put(4555,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4555,5380){\makebox(0,0){\strut{}Voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/vem0A3voronoiEOCH1-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/vem0A3voronoiEOCH2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(692,767){\makebox(0,0)[r]{\strut{}1.0}}%
      \csname LTb\endcsname%%
      \put(692,1257){\makebox(0,0)[r]{\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(692,1747){\makebox(0,0)[r]{\strut{}2.0}}%
      \csname LTb\endcsname%%
      \put(692,2237){\makebox(0,0)[r]{\strut{}2.5}}%
      \csname LTb\endcsname%%
      \put(692,2727){\makebox(0,0)[r]{\strut{}3.0}}%
      \csname LTb\endcsname%%
      \put(692,3218){\makebox(0,0)[r]{\strut{}3.5}}%
      \csname LTb\endcsname%%
      \put(692,3708){\makebox(0,0)[r]{\strut{}4.0}}%
      \csname LTb\endcsname%%
      \put(692,4198){\makebox(0,0)[r]{\strut{}4.5}}%
      \csname LTb\endcsname%%
      \put(692,4688){\makebox(0,0)[r]{\strut{}5.0}}%
      \csname LTb\endcsname%%
      \put(793,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(3301,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(5809,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(7517,4472){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(7517,4233){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(7517,3993){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(7517,3753){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ eoc}}}%
      \csname LTb\endcsname%%
      \put(4555,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4555,5380){\makebox(0,0){\strut{}Voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/vem0A3voronoiEOCH2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/vem0A3voronoiEOCL2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(692,767){\makebox(0,0)[r]{\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(692,1123){\makebox(0,0)[r]{\strut{}2.0}}%
      \csname LTb\endcsname%%
      \put(692,1480){\makebox(0,0)[r]{\strut{}2.5}}%
      \csname LTb\endcsname%%
      \put(692,1836){\makebox(0,0)[r]{\strut{}3.0}}%
      \csname LTb\endcsname%%
      \put(692,2193){\makebox(0,0)[r]{\strut{}3.5}}%
      \csname LTb\endcsname%%
      \put(692,2549){\makebox(0,0)[r]{\strut{}4.0}}%
      \csname LTb\endcsname%%
      \put(692,2906){\makebox(0,0)[r]{\strut{}4.5}}%
      \csname LTb\endcsname%%
      \put(692,3262){\makebox(0,0)[r]{\strut{}5.0}}%
      \csname LTb\endcsname%%
      \put(692,3619){\makebox(0,0)[r]{\strut{}5.5}}%
      \csname LTb\endcsname%%
      \put(692,3975){\makebox(0,0)[r]{\strut{}6.0}}%
      \csname LTb\endcsname%%
      \put(692,4332){\makebox(0,0)[r]{\strut{}6.5}}%
      \csname LTb\endcsname%%
      \put(692,4688){\makebox(0,0)[r]{\strut{}7.0}}%
      \csname LTb\endcsname%%
      \put(793,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(3301,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(5809,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(7517,4472){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(7517,4233){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(7517,3993){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(7517,3753){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ eoc}}}%
      \csname LTb\endcsname%%
      \put(4555,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4555,5380){\makebox(0,0){\strut{}Voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/vem0A3voronoiEOCL2-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/vem0A3voronoiEOCstar.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(692,767){\makebox(0,0)[r]{\strut{}1.0}}%
      \csname LTb\endcsname%%
      \put(692,1257){\makebox(0,0)[r]{\strut{}1.5}}%
      \csname LTb\endcsname%%
      \put(692,1747){\makebox(0,0)[r]{\strut{}2.0}}%
      \csname LTb\endcsname%%
      \put(692,2237){\makebox(0,0)[r]{\strut{}2.5}}%
      \csname LTb\endcsname%%
      \put(692,2727){\makebox(0,0)[r]{\strut{}3.0}}%
      \csname LTb\endcsname%%
      \put(692,3218){\makebox(0,0)[r]{\strut{}3.5}}%
      \csname LTb\endcsname%%
      \put(692,3708){\makebox(0,0)[r]{\strut{}4.0}}%
      \csname LTb\endcsname%%
      \put(692,4198){\makebox(0,0)[r]{\strut{}4.5}}%
      \csname LTb\endcsname%%
      \put(692,4688){\makebox(0,0)[r]{\strut{}5.0}}%
      \csname LTb\endcsname%%
      \put(793,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(3301,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(5809,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(7517,4472){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(7517,4233){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(7517,3993){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(7517,3753){\makebox(0,0)[r]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ eoc}}}%
      \csname LTb\endcsname%%
      \put(4555,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4555,5380){\makebox(0,0){\strut{}Voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/vem0A3voronoiEOCstar-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A3/eps/vem0A3voronoiErrstar.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(2825,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(4656,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(6487,527){\makebox(0,0){\strut{}$100000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$1\times10^{6}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}Voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A3/eps/vem0A3voronoiErrstar-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/H1A5-0.0125simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=$0.0125}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{eps/H1A5-0.0125simplexEOC}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/H1A5-0.025simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=$0.025}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{eps/H1A5-0.025simplexEOC}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/H1A5-0.05simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,1551){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2335){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3120){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,3904){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=$0.05}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{eps/H1A5-0.05simplexEOC}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/H1A5-0.1simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1551){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2335){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3120){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3904){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=$0.1}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{eps/H1A5-0.1simplexEOC}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/H1A5-0125simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=0.0125$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5a/eps/H1A5-0125simplexEOC-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/H1A5-025simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=0.025$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5a/eps/H1A5-025simplexEOC-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/H1A5-05simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,1551){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2335){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3120){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,3904){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=0.05$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5a/eps/H1A5-05simplexEOC-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/H1A5-1simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1551){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2335){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3120){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3904){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=0.1$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5a/eps/H1A5-1simplexEOC-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/H2A5-0.0125simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+03}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=$0.0125}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{eps/H2A5-0.0125simplexEOC}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/H2A5-0.025simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+03}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=$0.025}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{eps/H2A5-0.025simplexEOC}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/H2A5-0.05simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=$0.05}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{eps/H2A5-0.05simplexEOC}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/H2A5-0.1simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=$0.1}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{eps/H2A5-0.1simplexEOC}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/H2A5-0125simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+03}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=0.0125$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5a/eps/H2A5-0125simplexEOC-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/H2A5-025simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+03}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=0.025$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5a/eps/H2A5-025simplexEOC-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/H2A5-05simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=0.05$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5a/eps/H2A5-05simplexEOC-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/H2A5-1simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=0.1$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5a/eps/H2A5-1simplexEOC-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/L2A5-0.0125simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=$0.0125}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{eps/L2A5-0.0125simplexEOC}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/L2A5-0.025simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1551){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2335){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3120){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3904){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=$0.025}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{eps/L2A5-0.025simplexEOC}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/L2A5-0.05simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1551){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2335){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3120){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3904){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=$0.05}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{eps/L2A5-0.05simplexEOC}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/L2A5-0.1simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=$0.1}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{eps/L2A5-0.1simplexEOC}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/L2A5-0125simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=0.0125$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5a/eps/L2A5-0125simplexEOC-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/L2A5-025simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,1551){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,2335){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3120){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3904){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=0.025$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5a/eps/L2A5-025simplexEOC-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/L2A5-05simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1551){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2335){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3120){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,3904){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=0.05$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5a/eps/L2A5-05simplexEOC-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/L2A5-1simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-07}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=0.1$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5a/eps/L2A5-1simplexEOC-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/starA5-0.0125simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+03}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=$0.0125}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{eps/starA5-0.0125simplexEOC}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/starA5-0.025simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+03}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=$0.025}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{eps/starA5-0.025simplexEOC}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/starA5-0.05simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=$0.05}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{eps/starA5-0.05simplexEOC}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/starA5-0.1simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=$0.1}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{eps/starA5-0.1simplexEOC}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/starA5-0125simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+03}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=0.0125$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5a/eps/starA5-0125simplexEOC-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/starA5-025simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+03}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=0.025$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5a/eps/starA5-025simplexEOC-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/starA5-05simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=0.05$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5a/eps/starA5-05simplexEOC-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5a/eps/starA5-1simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,1747){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,3708){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,2181){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM-Weak}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=0.1$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5a/eps/starA5-1simplexEOC-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5b/eps/H1A5-05simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,1617){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2468){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,3319){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,4170){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,5020){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2893){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^1$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=0.05$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5b/eps/H1A5-05simplexEOC-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5b/eps/H2A5-05simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,2184){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,3602){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,5020){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2893){\rotatebox{-270.00}{\makebox(0,0){\strut{}$H^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=0.05$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5b/eps/H2A5-05simplexEOC-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5b/eps/L2A5-05simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-06}}%
      \csname LTb\endcsname%%
      \put(894,1617){\makebox(0,0)[r]{\strut{}1e-05}}%
      \csname LTb\endcsname%%
      \put(894,2468){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,3319){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,4170){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,5020){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2893){\rotatebox{-270.00}{\makebox(0,0){\strut{}$L^2$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=0.05$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5b/eps/L2A5-05simplexEOC-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5b/eps/starA5-0125simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,2893){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(894,5020){\makebox(0,0)[r]{\strut{}1e+03}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2893){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=0.0125$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5b/eps/starA5-0125simplexEOC-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5b/eps/starA5-05simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,2184){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,3602){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,5020){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2893){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=0.05$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5b/eps/starA5-05simplexEOC-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5b/eps/starA5-1simplexEOC.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,1830){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,2893){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,3957){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,5020){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,1941){\makebox(0,0)[l]{\strut{}VEM(m,m,m)}}%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m-1,m-1,m-1)}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m-2,m-2,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m-1,m-2)}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}DG}}%
      \csname LTb\endcsname%%
      \put(195,2893){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}m=4, $delta=0.1$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5b/eps/starA5-1simplexEOC-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5b/eps/vem0A5-0.0125simplex_20.tex <==
\begin{tabular}{rrr}
\hline
   $H^2$ &   $H^1$ &   $L^2$ \\
\hline
    0.13 &    0.45 &    0.88 \\
    0.31 &    0.71 &    1.03 \\
    0.53 &    0.96 &    1.27 \\
    0.69 &    1.2  &    1.54 \\
\hline
\end{tabular}

==> results/A5b/eps/vem0A5-0.0125simplex_30.tex <==
\begin{tabular}{rrr}
\hline
   $H^2$ &   $H^1$ &   $L^2$ \\
\hline
    0.59 &    1.14 &    1.93 \\
    1.04 &    1.75 &    2.6  \\
    1.24 &    2.01 &    2.82 \\
\hline
\end{tabular}

==> results/A5b/eps/vem0A5-0.0125simplex_40.tex <==
\begin{tabular}{rrr}
\hline
   $H^2$ &   $H^1$ &   $L^2$ \\
\hline
    0.7  &    1.23 &    1.92 \\
    1.36 &    2.06 &    2.9  \\
    2.12 &    2.96 &    3.85 \\
\hline
\end{tabular}

==> results/A5b/eps/vem0A5-0.0125simplex_50.tex <==
\begin{tabular}{rrr}
\hline
   $H^2$ &   $H^1$ &   $L^2$ \\
\hline
    1.23 &    1.86 &    2.52 \\
    2.14 &    2.91 &    3.72 \\
\hline
\end{tabular}

==> results/A5b/eps/vem0A5-0.0125voronoi_20.tex <==
\begin{tabular}{rrr}
\hline
   $H^2$ &   $H^1$ &   $L^2$ \\
\hline
    0.06 &    0.26 &    0.58 \\
    0.08 &    0.25 &    0.52 \\
    0.16 &    0.37 &    0.68 \\
    0.22 &    0.48 &    0.81 \\
\hline
\end{tabular}

==> results/A5b/eps/vem0A5-0.0125voronoi_30.tex <==
\begin{tabular}{rrr}
\hline
   $H^2$ &   $H^1$ &   $L^2$ \\
\hline
    0.36 &    0.79 &    1.33 \\
    0.46 &    0.8  &    1.22 \\
    1    &    1.53 &    2.05 \\
    1.14 &    1.69 &    2.26 \\
\hline
\end{tabular}

==> results/A5b/eps/vem0A5-0.0125voronoi_40.tex <==
\begin{tabular}{rrr}
\hline
   $H^2$ &   $H^1$ &   $L^2$ \\
\hline
    0.85 &    1.41 &    2.06 \\
    1.56 &    2.11 &    2.53 \\
    2.61 &    3.39 &    4.11 \\
\hline
\end{tabular}

==> results/A5b/eps/vem0A5-0.0125voronoi_50.tex <==
\begin{tabular}{rrr}
\hline
   $H^2$ &   $H^1$ &   $L^2$ \\
\hline
    1.76 &    2.51 &    3.28 \\
    2.75 &    3.37 &    3.95 \\
\hline
\end{tabular}

==> results/A5b/eps/vem0A5-0.1simplexErrstar.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,1551){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,2335){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,3120){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,3904){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}Simplex grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5b/eps/vem0A5-0.1simplexErrstar-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> results/A5b/eps/vem0A5-0.1voronoiErrstar.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(8640.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(894,767){\makebox(0,0)[r]{\strut{}1e-04}}%
      \csname LTb\endcsname%%
      \put(894,1420){\makebox(0,0)[r]{\strut{}1e-03}}%
      \csname LTb\endcsname%%
      \put(894,2074){\makebox(0,0)[r]{\strut{}1e-02}}%
      \csname LTb\endcsname%%
      \put(894,2727){\makebox(0,0)[r]{\strut{}1e-01}}%
      \csname LTb\endcsname%%
      \put(894,3381){\makebox(0,0)[r]{\strut{}1e+00}}%
      \csname LTb\endcsname%%
      \put(894,4035){\makebox(0,0)[r]{\strut{}1e+01}}%
      \csname LTb\endcsname%%
      \put(894,4688){\makebox(0,0)[r]{\strut{}1e+02}}%
      \csname LTb\endcsname%%
      \put(994,527){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%%
      \put(3435,527){\makebox(0,0){\strut{}$1000$}}%
      \csname LTb\endcsname%%
      \put(5876,527){\makebox(0,0){\strut{}$10000$}}%
      \csname LTb\endcsname%%
      \put(8317,527){\makebox(0,0){\strut{}$100000$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1795,1701){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=2}}%
      \csname LTb\endcsname%%
      \put(1795,1462){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=3}}%
      \csname LTb\endcsname%%
      \put(1795,1222){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=4}}%
      \csname LTb\endcsname%%
      \put(1795,982){\makebox(0,0)[l]{\strut{}VEM(m,m,m) m=5}}%
      \csname LTb\endcsname%%
      \put(195,2727){\rotatebox{-270.00}{\makebox(0,0){\strut{}$\|\cdot\|_\star$ error}}}%
      \csname LTb\endcsname%%
      \put(4656,167){\makebox(0,0){\strut{}number of dofs}}%
      \csname LTb\endcsname%%
      \put(4656,5380){\makebox(0,0){\strut{}Voronoi grid}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={432.00bp},height={288.00bp}]{results/A5b/eps/vem0A5-0.1voronoiErrstar-pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup

